BIAS: A Body-based Interpretable Active Speaker Approach

State-of-the-art Active Speaker Detection (ASD) approaches heavily rely on audio and facial features to perform, which is not a sustainable approach in wild scenarios. Although these methods achieve good results in the standard AVA-ActiveSpeaker set, a recent wilder ASD dataset (WASD) showed the limitations of such models and raised the need for new approaches. As such, we propose BIAS, a model that, for the first time, combines audio, face, and body information, to accurately predict active speakers in varying/challenging conditions. Additionally, we design BIAS to provide interpretability by proposing a novel use for Squeeze-and-Excitation blocks, namely in attention heatmaps creation and feature importance assessment. For a full interpretability setup, we annotate an ASD-related actions dataset (ASD-Text) to finetune a ViT-GPT2 for text scene description to complement BIAS interpretability. The results show that BIAS is state-of-the-art in challenging conditions where body-based features are of utmost importance (Columbia, open-settings, and WASD), and yields competitive results in AVA-ActiveSpeaker, where face is more influential than body for ASD. BIAS interpretability also shows the features/aspects more relevant towards ASD prediction in varying settings, making it a strong baseline for further developments in interpretable ASD models, and is available at https://github.com/Tiago-Roxo/BIAS.

==> article/biographies.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Tiago_Roxo.png}}]{Tiago Roxo} obtained a bachelor's degree in Computer Science and Engineering from Universidade da Beira Interior (UBI) in 2019 and is currently pursuing a Ph.D.'s degree, with a FCT (\textit{Funda\c{c}\~{a}o para a Ciência e a Tecnologia}) scholarship, in the field of Computer Vision and Artificial Intelligence.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/joana_costa.png}}]{Joana C. Costa} obtained her bachelor's and master's degree in Computer Science and Engineering from Universidade da Beira Interior (UBI) in 2019 and 2021, respectively. She is currently pursuing a Ph.D.'s degree, with a FCT (\textit{Funda\c{c}\~{a}o para a Ciência e a Tecnologia}) scholarship, in the field of Computer Vision and Adversarial Attacks.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Pedro_Inacio.png}}]{Pedro R. M. In\'{a}cio} was born in Covilh\~{a}, Portugal, in 1982. Holds a 5-year B.Sc. degree in Mathematics/Computer Science and a Ph.D. degree in Computer Science and Engineering, obtained from the Universidade da Beira Interior (UBI), Portugal, in 2005 and 2009 respectively. The Ph.D. work was performed in the enterprise environment of Nokia Siemens Networks Portugal S.A., through a Ph.D. grant from the Portuguese Foundation for Science and Technology.

He is a professor of Computer Science at UBI since 2010, where he lectures subjects related with information assurance and security, programming of mobile devices and computer based simulation, to graduate and undergraduate courses, namely to the B.Sc., M.Sc. and Ph.D. programmes in Computer Science and Engineering. He is currently the Head of the Department of Computer Science of UBI. He is an instructor of the UBI Cisco Academy.

He is an IEEE senior member and a researcher of the Instituto de Telecomunica\c{c}\~{o}es (IT). His main research topics are information assurance and security, computer based simulation, and network traffic monitoring, analysis and classification. He has about 40 publications in the form of book chapters and papers in international peer-reviewed books, conferences and journals. He frequently reviews papers for IEEE, Springer, Wiley and Elsevier journals. He has been member of the Technical Program Committee of international conferences such as the ACM Symposium on Applied Computing - Track on Networking. He was one of the chairs of WISARC 2016.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Hugo_Proenca.pdf}}]{Hugo Proen\c{c}a} (SM'12), B.Sc. (2001), M.Sc. (2004) and Ph.D. (2007) is an Associate Professor in the Department of Computer Science, University of Beira Interior and has been researching mainly about biometrics and visual-surveillance. He was the coordinating editor of the IEEE Biometrics Council Newsletter and the area editor (ocular biometrics) of the IEEE Biometrics Compendium Journal. He is a member of the Editorial Boards of the Image and Vision Computing, IEEE Access and International Journal of Biometrics. Also, he served as Guest Editor of special issues of the Pattern Recognition Letters, Image and Vision Computing and Signal, Image and Video Processing journals. 
\end{IEEEbiography}
